Embodied Supervision: Haptic Display of Automation Command to Improve Supervisory Performance

A human operator using a manual control interface has ready access to their own command signal, both by efference copy and proprioception. In contrast, a human supervisor typically relies on visual information alone. We propose supplying a supervisor with a copy of the operators command signal, hypothesizing improved performance, especially when that copy is provided through haptic display. We experimentally compared haptic with visual access to the command signal, quantifying the performance of N equals 10 participants attempting to determine which of three reference signals was being tracked by an operator. Results indicate an improved accuracy in identifying the tracked target when haptic display was available relative to visual display alone. We conjecture the benefit follows from the relationship of haptics to the supervisor's own experience, perhaps muscle memory, as an operator.

==> references.tex <==
@article{mcruer1965human,
  title={Human pilot dynamics in compensatory systems-theory, models, and experiments with controlled element and forcing function variations},
  author={McRuer, Duane T},
  journal={AFFDL-TR-65-15},
  year={1965}
}

@article{optcon,
  title={An Optimal Control Model of Human Response Part I: Theory and Validation},
  author={Kleinman, D. L. and Baron, S. and Levison, W. H.},
  journal={Automatica},
  year={1970}
}
@article{bridgeman2007efference,
  title={Efference copy and its limitations},
  author={Bridgeman, Bruce},
  journal={Computers in biology and medicine},
  volume={37},
  number={7},
  pages={924--929},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{gold2013take,
  title={“Take over!” How long does it take to get the driver back into the loop?},
  author={Gold, Christian and Damb{\"o}ck, Daniel and Lorenz, Lutz and Bengler, Klaus},
  booktitle={Proceedings of the human factors and ergonomics society annual meeting},
  volume={57},
  number={1},
  pages={1938--1942},
  year={2013},
  organization={Sage Publications Sage CA: Los Angeles, CA}
}
@article{merat2012highly,
  title={Highly automated driving, secondary task performance, and driver state},
  author={Merat, Natasha and Jamson, A Hamish and Lai, Frank CH and Carsten, Oliver},
  journal={Human factors},
  volume={54},
  number={5},
  pages={762--771},
  year={2012},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{parasuraman2008situation,
  title={Situation awareness, mental workload, and trust in automation: Viable, empirically supported cognitive engineering constructs},
  author={Parasuraman, Raja and Sheridan, Thomas B and Wickens, Christopher D},
  journal={Journal of cognitive engineering and decision making},
  volume={2},
  number={2},
  pages={140--160},
  year={2008},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{jablonowski2020beyond,
  title={Beyond drone vision: the embodied telepresence of first-person-view drone flight},
  author={Jablonowski, Maximilian},
  journal={The Senses and Society},
  volume={15},
  number={3},
  pages={344--358},
  year={2020},
  publisher={Taylor \& Francis}
}

% Supervision
%Defines human as supervisor
@incollection{sheridan1988task,
  title={Task allocation and supervisory control},
  author={Sheridan, Thomas B},
  booktitle={Handbook of human-computer interaction},
  pages={159--173},
  year={1988},
  publisher={Elsevier}
}
@article{hong2017multimodal,
  title={Multimodal feedback for teleoperation of multiple mobile robots in an outdoor environment},
  author={Hong, Ayoung and Lee, Dong Gun and B{\"u}lthoff, Heinrich H and Son, Hyoung Il},
  journal={Journal on Multimodal User Interfaces},
  volume={11},
  pages={67--80},
  year={2017},
  publisher={Springer}
}

@inproceedings{schmidt2015tactile,
  title={Tactile Feedback and Situation Awareness-Improving Adherence to an Envelope in Sidestick-Controlled Fly-by-Wire Aircrafts},
  author={Schmidt-Skipiol, Florian J and Hecker, Peter},
  booktitle={15th AIAA Aviation Technology, Integration, and Operations Conference},
  pages={2905},
  year={2015}
}
@article{chen2010supervisory,
  title={Supervisory control of multiple robots: Human-performance issues and user-interface design},
  author={Chen, Jessie YC and Barnes, Michael J and Harper-Sciarini, Michelle},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
  volume={41},
  number={4},
  pages={435--454},
  year={2010},
  publisher={IEEE}
}
% Demonstrates intent improves mental model of system
@inproceedings{furukawa2003supporting,
  title={Supporting system-centered view of operators through ecological interface design: Two experiments on human-centered automation},
  author={Furukawa, Hiroshi and Parasuraman, Raja},
  booktitle={Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
  volume={47},
  number={3},
  pages={567--571},
  year={2003},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}
@article{furukawa2005intention,
  title={Intention-represented ecological interface design for supporting collaboration with automation: Situation awareness and control in inexperienced scenarios},
  author={Furukawa, Hiroshi and Nakatani, Hiroyuki and Inagaki, Toshiyuki},
  journal={Human Performance, Situation Awareness, and Automation: Current Research and Trends HPSAA II, Volumes I and II},
  pages={49},
  year={2005},
  publisher={Psychology Press}
}
@article{aarts2005inference,
  title={On the inference of personal authorship: Enhancing experienced agency by priming effect information},
  author={Aarts, Henk and Custers, Ruud and Wegner, Daniel M},
  journal={Consciousness and cognition},
  volume={14},
  number={3},
  pages={439--458},
  year={2005},
  publisher={Elsevier}
}
%prediction in situational awareness
@article{roldan2017multi,
  title={Multi-robot interfaces and operator situational awareness: Study of the impact of immersion and prediction},
  author={Rold{\'a}n, Juan Jes{\'u}s and Pe{\~n}a-Tapia, Elena and Mart{\'\i}n-Barrio, Andr{\'e}s and Olivares-M{\'e}ndez, Miguel A and Del Cerro, Jaime and Barrientos, Antonio},
  journal={Sensors},
  volume={17},
  number={8},
  pages={1720},
  year={2017},
  publisher={MDPI}
}

% Multiple cameras
% Camera coordination for HRI
@article{recchiuto2016visual,
  title={Visual feedback with multiple cameras in a UAVs Human--Swarm Interface},
  author={Recchiuto, Carmine Tommaso and Sgorbissa, Antonio and Zaccaria, Renato},
  journal={Robotics and Autonomous Systems},
  volume={80},
  pages={43--54},
  year={2016},
  publisher={Elsevier}
}


% temporal predictability
% New additions
% related topic gaining traction --- sense of agency

@article{mulliken2008forward,
  title={Forward estimation of movement state in posterior parietal cortex},
  author={Mulliken, Grant H and Musallam, Sam and Andersen, Richard A},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={24},
  pages={8170--8177},
  year={2008},
  publisher={National Acad Sciences}
}
@article{ikegami2017shared,
  title={Shared mechanisms in the estimation of self-generated actions and the prediction of other’s actions by humans},
  author={Ikegami, Tsuyoshi and Ganesh, Gowrishankar},
  journal={eneuro},
  volume={4},
  number={6},
  year={2017},
  publisher={Society for Neuroscience}
}

@article{imamizu2010prediction,
  title={Prediction of sensorimotor feedback from the efference copy of motor commands: A review of behavioral and functional neuroimaging studies},
  author={Imamizu, Hiroshi},
  journal={Japanese Psychological Research},
  volume={52},
  number={2},
  pages={107--120},
  year={2010},
  publisher={Wiley Online Library}
}
@article{adams2013predictions,
  title={Predictions not commands: active inference in the motor system},
  author={Adams, Rick A and Shipp, Stewart and Friston, Karl J},
  journal={Brain Structure and Function},
  volume={218},
  pages={611--643},
  year={2013},
  publisher={Springer}
}

@article{haggard2005conscious,
  title={Conscious intention and motor cognition},
  author={Haggard, Patrick},
  journal={Trends in cognitive sciences},
  volume={9},
  number={6},
  pages={290--295},
  year={2005},
  publisher={Elsevier}
}
@article{hapuarachchi2022knowing,
  title={Knowing the intention behind limb movements of a partner increases embodiment towards the limb of joint avatar},
  author={Hapuarachchi, Harin and Kitazaki, Michiteru},
  journal={Scientific Reports},
  volume={12},
  number={1},
  pages={11453},
  year={2022},
  publisher={Nature Publishing Group UK London}
}

@article{rineau2023being,
  title={Being active over one’s own motion: Considering predictive mechanisms in self-motion perception},
  author={Rineau, Anne-Laure and Bringoux, Lionel and Sarrazin, Jean-Christophe and Berberian, Bruno},
  journal={Neuroscience \& Biobehavioral Reviews},
  pages={105051},
  year={2023},
  publisher={Elsevier}
}
@article{mccord1991input,
  title={Input-versus output-oriented instructions on a compensatory tracking task: support for control theory},
  author={McCord, David M},
  journal={The Psychological Record},
  volume={41},
  pages={401--413},
  year={1991},
  publisher={Springer}
}




@article{shanechi2012feedback,
  title={Feedback-controlled parallel point process filter for estimation of goal-directed movements from neural signals},
  author={Shanechi, Maryam M and Wornell, Gregory W and Williams, Ziv M and Brown, Emery N},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={21},
  number={1},
  pages={129--140},
  year={2012},
  publisher={IEEE}
}


% vision 
@inproceedings{li2015flying,
  title={Flying frustum: A spatial interface for enhancing human-uav awareness},
  author={Li, Nico and Cartwright, Stephen and Shekhar Nittala, Aditya and Sharlin, Ehud and Costa Sousa, Mario},
  booktitle={Proceedings of the 3rd International Conference on Human-Agent Interaction},
  pages={27--31},
  year={2015}
}

% haptic feedback
@inproceedings{zhang2021haptic,
  title={Haptic feedback improves human-robot agreement and user satisfaction in shared-autonomy teleoperation},
  author={Zhang, Dawei and Tron, Roberto and Khurshid, Rebecca P},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3306--3312},
  year={2021},
  organization={IEEE}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Evidence that haptic feedback supplies intent in shared control 
%nice old paper of yours that talks about this transference of intent
@article{griffiths2005sharing,
  title={Sharing control between humans and automation using haptic interface: Primary and secondary task performance benefits},
  author={Griffiths, Paul G and Gillespie, R Brent},
  journal={Human factors},
  volume={47},
  number={3},
  pages={574--590},
  year={2005},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{nishimura2015haptic,
  title={Haptic shared control in steering operation based on cooperative status between a driver and a driver assistance system},
  author={Nishimura, Ryota and Wada, Takahiro and Sugiyama, Seiji},
  journal={arXiv preprint arXiv:1504.05770},
  year={2015}
}

@article{cutlip2021effects,
  title={The effects of haptic feedback and transition type on transfer of control between drivers and vehicle automation},
  author={Cutlip, Steven and Wan, Yuzhi and Sarter, Nadine and Gillespie, R Brent},
  journal={IEEE Transactions on Human-Machine Systems},
  volume={51},
  number={6},
  pages={613--621},
  year={2021},
  publisher={IEEE}
}


% temporal prediction
@article{hughes2013mechanisms,
  title={Mechanisms of intentional binding and sensory attenuation: the role of temporal prediction, temporal control, identity prediction, and motor prediction.},
  author={Hughes, Gethin and Desantis, Andrea and Waszak, Florian},
  journal={Psychological bulletin},
  volume={139},
  number={1},
  pages={133},
  year={2013},
  publisher={American Psychological Association}
}
@article{desantis2014temporal,
  title={The temporal dynamics of the perceptual consequences of action-effect prediction},
  author={Desantis, Andrea and Roussel, Cedric and Waszak, Florian},
  journal={Cognition},
  volume={132},
  number={3},
  pages={243--250},
  year={2014},
  publisher={Elsevier}
}

@incollection{bainbridge1983ironies,
  title={Ironies of automation},
  author={Bainbridge, Lisanne},
  booktitle={Analysis, design and evaluation of man--machine systems},
  pages={129--135},
  year={1983},
  publisher={Elsevier}
}

@article{sheridan2012human,
  title={Human supervisory control},
  author={Sheridan, Thomas B},
  journal={Handbook of human factors and ergonomics},
  pages={990--1015},
  year={2012},
  publisher={Wiley Online Library}
}

@article{sheridan2016human,
  title={Human--robot interaction: status and challenges},
  author={Sheridan, Thomas B},
  journal={Human factors},
  volume={58},
  number={4},
  pages={525--532},
  year={2016},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{von1971principle,
  title={The principle of reafference: Interactions between the central nervous system and the peripheral organs},
  author={von Holst, Erich and Mittelstaedt, Horst},
  journal={Perceptual processing: Stimulus equivalence and pattern recognition},
  pages={41--72},
  year={1971},
  publisher={Appleton New York}
}

@article{jeannerod2003action,
  title={Action monitoring and forward control of movements},
  author={Jeannerod, M and Arbib, Michael},
  journal={The handbook of brain theory and neural networks},
  pages={83--85},
  year={2003},
  publisher={MIT Press Cambridge, MA}
}

@article{miall1993cerebellum,
  title={Is the cerebellum a smith predictor?},
  author={Miall, R Christopher and Weir, D Jo and Wolpert, Daniel M and Stein, JF},
  journal={Journal of motor behavior},
  volume={25},
  number={3},
  pages={203--216},
  year={1993},
  publisher={Taylor \& Francis}
}

@article{cao2022optimal,
  title={Optimal Estimation with Sensor Delay},
  author={Cao, Di and Cowan, Noah J and Freudenberg, James S},
  journal={arXiv preprint arXiv:2210.12123},
  year={2022}
}

@article{storms2017shared,
  title={A shared control method for obstacle avoidance with mobile robots and its interaction with communication delay},
  author={Storms, Justin and Chen, Kevin and Tilbury, Dawn},
  journal={The International Journal of Robotics Research},
  volume={36},
  number={5-7},
  pages={820--839},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{storms2014predicting,
  title={Predicting human performance during teleoperation},
  author={Storms, Justin and Vozar, Steven and Tilbury, Dawn},
  booktitle={Proceedings of the 2014 ACM/IEEE international conference on Human-robot interaction},
  pages={298--299},
  year={2014}
}

@article{tsutsui2003effect,
  title={Effect of manual guidance on acquiring a new bimanual coordination pattern},
  author={Tsutsui, Seijiro and Imanaka, Kuniyasu},
  journal={Research quarterly for exercise and sport},
  volume={74},
  number={1},
  pages={104--109},
  year={2003},
  publisher={Taylor \& Francis}
}

@article{mcruer1967review,
  title={A review of quasi-linear pilot models},
  author={McRuer, Duane T and Jex, Henry R},
  journal={IEEE transactions on human factors in electronics},
  number={3},
  pages={231--249},
  year={1967},
  publisher={IEEE}
}

@inproceedings{mcruer1974mathematical,
  title={Mathematical models of human pilot behavior},
  author={McRuer, Duane T and Krendel, Ezra S},
  year={1974},
  organization={AGARD}
}

@inproceedings{cutlip2019haptic,
  title={Haptic feedback and the internal model principle},
  author={Cutlip, Steven and Freudenberg, Jim and Cowan, Noah and Gillespie, R Brent},
  booktitle={2019 IEEE World Haptics Conference (WHC)},
  pages={568--573},
  year={2019},
  organization={IEEE}
}

@article{miall1995cerebellum,
  title={The cerebellum as a predictive model of the motor system: a Smith Predictor hypothesis},
  author={Miall, RC and Wolpert, DM},
  journal={Neural control of movement},
  pages={215--223},
  year={1995},
  publisher={Springer}
}

@inproceedings{thompson1988comparison,
  title={Comparison of the human optimal control and crossover models},
  author={THOMPSON, PETER and MCRUER, DUANE},
  booktitle={Guidance, Navigation and Control Conference},
  pages={4183},
  year={1988}
}

@article{mcruer1968neuromuscular,
  title={A neuromuscular actuation system model},
  author={McRuer, Duane T and Magdaleno, Raymond E and Moore, George P},
  journal={IEEE Transactions on Man-Machine Systems},
  volume={9},
  number={3},
  pages={61--71},
  year={1968},
  publisher={IEEE}
}

@inproceedings{boelhouwer2019turmoil,
  title={Turmoil behind the automated wheel: an embodied perspective on current HMI developments in partially automated vehicles},
  author={Boelhouwer, Anika and van Dijk, Jelle and Martens, Marieke H},
  booktitle={HCI in Mobility, Transport, and Automotive Systems: First International Conference, MobiTAS 2019, Held as Part of the 21st HCI International Conference, HCII 2019, Orlando, FL, USA, July 26-31, 2019, Proceedings 21},
  pages={3--25},
  year={2019},
  organization={Springer}
}

@article{abbink2012haptic,
  title={Haptic shared control: smoothly shifting control authority?},
  author={Abbink, David A and Mulder, Mark and Boer, Erwin R},
  journal={Cognition, Technology \& Work},
  volume={14},
  pages={19--28},
  year={2012},
  publisher={Springer}
}
@article{kleinman1970optimal,
  title={An optimal control model of human response part I: Theory and validation},
  author={Kleinman, David L and Baron, S and Levison, WH},
  journal={Automatica},
  volume={6},
  number={3},
  pages={357--369},
  year={1970},
  publisher={Elsevier}
}

@article{rolnick1991driver,
  title={Why is the driver rarely motion sick? The role of controllability in motion sickness},
  author={Rolnick, Arnon and Lubow, RE},
  journal={Ergonomics},
  volume={34},
  number={7},
  pages={867--879},
  year={1991},
  publisher={Taylor \& Francis}
}
% Human Supervision

@article{al2019alert,
  title={An alert-generation framework for improving resiliency in human-supervised, multi-agent teams},
  author={Al-Hussaini, Sarah and Gregory, Jason M and Shriyam, Shaurya and Gupta, Satyandra K},
  journal={arXiv preprint arXiv:1909.06480},
  year={2019}
}

%Defines human as supervisor
@incollection{sheridan1988task,
  title={Task allocation and supervisory control},
  author={Sheridan, Thomas B},
  booktitle={Handbook of human-computer interaction},
  pages={159--173},
  year={1988},
  publisher={Elsevier}
}




% Review Papers

@article{sheridan2016human,
  title={Human--robot interaction: status and challenges},
  author={Sheridan, Thomas B},
  journal={Human factors},
  volume={58},
  number={4},
  pages={525--532},
  year={2016},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{sheridan2021human,
  title={Human supervisory control of automation},
  author={Sheridan, Thomas B},
  journal={Handbook of Human Factors and Ergonomics},
  pages={736--760},
  year={2021},
  publisher={Wiley Online Library}
}


% Situational Awareness
@article{parasuraman2008situation,
  title={Situation awareness, mental workload, and trust in automation: Viable, empirically supported cognitive engineering constructs},
  author={Parasuraman, Raja and Sheridan, Thomas B and Wickens, Christopher D},
  journal={Journal of cognitive engineering and decision making},
  volume={2},
  number={2},
  pages={140--160},
  year={2008},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{hong2017multimodal,
  title={Multimodal feedback for teleoperation of multiple mobile robots in an outdoor environment},
  author={Hong, Ayoung and Lee, Dong Gun and B{\"u}lthoff, Heinrich H and Son, Hyoung Il},
  journal={Journal on Multimodal User Interfaces},
  volume={11},
  pages={67--80},
  year={2017},
  publisher={Springer}
}

@inproceedings{schmidt2015tactile,
  title={Tactile Feedback and Situation Awareness-Improving Adherence to an Envelope in Sidestick-Controlled Fly-by-Wire Aircrafts},
  author={Schmidt-Skipiol, Florian J and Hecker, Peter},
  booktitle={15th AIAA Aviation Technology, Integration, and Operations Conference},
  pages={2905},
  year={2015}
}
% Task switching for supervision
@article{mcfarlane2002scope,
  title={The scope and importance of human interruption in human-computer interaction design},
  author={McFarlane, Daniel C and Latorella, Kara A},
  journal={Human-Computer Interaction},
  volume={17},
  number={1},
  pages={1--61},
  year={2002},
  publisher={Taylor \& Francis}
}





% Survey paper with compensatory control 
@article{scibilia2022human,
  title={Human control model estimation in physical human--machine interaction: A survey},
  author={Scibilia, Adriano and Pedrocchi, Nicola and Fortuna, Luigi},
  journal={Sensors},
  volume={22},
  number={5},
  pages={1732},
  year={2022},
  publisher={MDPI}
}

% feedforward to suppliment feedback, uses McRuer's crossover model to model human's response in compensatory control
@article{drop2013identification,
  title={Identification of the feedforward component in manual control with predictable target signals},
  author={Drop, Frank M and Pool, Daan M and Damveld, Herman J and van Paassen, Marinus M and Mulder, Max},
  journal={IEEE transactions on cybernetics},
  volume={43},
  number={6},
  pages={1936--1949},
  year={2013},
  publisher={IEEE}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Supervisory Control
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{chen2010supervisory,
  title={Supervisory control of multiple robots: Human-performance issues and user-interface design},
  author={Chen, Jessie YC and Barnes, Michael J and Harper-Sciarini, Michelle},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
  volume={41},
  number={4},
  pages={435--454},
  year={2010},
  publisher={IEEE}
}

@inproceedings{kurowski2016online,
  title={Online interaction of a human supervisor with multi-robot task allocation},
  author={Kurowski, Karen and von Stryk, Oskar},
  booktitle={Intelligent Autonomous Systems 13: Proceedings of the 13th International Conference IAS-13},
  pages={965--978},
  year={2016},
  organization={Springer}
}

@inproceedings{liu2015supervisory,
  title={A supervisory control method for multi-robot task allocation in urban search and rescue},
  author={Liu, Yugang and Ficocelli, Maurizio and Nejat, Goldie},
  booktitle={2015 IEEE International Symposium on Safety, Security, and Rescue Robotics (SSRR)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

% Camera coordination for HRI
@article{recchiuto2016visual,
  title={Visual feedback with multiple cameras in a UAVs Human--Swarm Interface},
  author={Recchiuto, Carmine Tommaso and Sgorbissa, Antonio and Zaccaria, Renato},
  journal={Robotics and Autonomous Systems},
  volume={80},
  pages={43--54},
  year={2016},
  publisher={Elsevier}
}



% Similar to  human preference in task assignment idea
@inproceedings{kurowski2016online,
  title={Online interaction of a human supervisor with multi-robot task allocation},
  author={Kurowski, Karen and von Stryk, Oskar},
  booktitle={Intelligent Autonomous Systems 13: Proceedings of the 13th International Conference IAS-13},
  pages={965--978},
  year={2016},
  organization={Springer}
}



% Improving situational awareness with vr

@article{roldan2017multi,
  title={Multi-robot interfaces and operator situational awareness: Study of the impact of immersion and prediction},
  author={Rold{\'a}n, Juan Jes{\'u}s and Pe{\~n}a-Tapia, Elena and Mart{\'\i}n-Barrio, Andr{\'e}s and Olivares-M{\'e}ndez, Miguel A and Del Cerro, Jaime and Barrientos, Antonio},
  journal={Sensors},
  volume={17},
  number={8},
  pages={1720},
  year={2017},
  publisher={MDPI}
}


%Similar to what I wanted to do with task assignment
@article{al2023generating,
  title={Generating Task Reallocation Suggestions to Handle Contingencies in Human-Supervised Multi-Robot Missions},
  author={Al-Hussaini, Sarah and Gregory, Jason M and Gupta, Satyandra K},
  journal={IEEE Transactions on Automation Science and Engineering},
  year={2023},
  publisher={IEEE}
}

@article{kelleyhuman,
  title={On Human-Assisted Multiagent-Based Planning},
  author={Kelley, Leah and Ouimet, Michael}
}

% Describes feelings of first person perspective drone flying
@article{jablonowski2020beyond,
  title={Beyond drone vision: the embodied telepresence of first-person-view drone flight},
  author={Jablonowski, Maximilian},
  journal={The Senses and Society},
  volume={15},
  number={3},
  pages={344--358},
  year={2020},
  publisher={Taylor \& Francis}
}

% Drone supervisory control
@inproceedings{bevacqua2015mixed,
  title={Mixed-initiative planning and execution for multiple drones in search and rescue missions},
  author={Bevacqua, Giuseppe and Cacace, Jonathan and Finzi, Alberto and Lippiello, Vincenzo},
  booktitle={Proceedings of the International Conference on Automated Planning and Scheduling},
  volume={25},
  pages={315--323},
  year={2015}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Human as observer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Equations for human as observer relating to intake of visual information
@article{senders1964human,
  title={The human operator as a monitor and controller of multidegree of freedom systems},
  author={Senders, John W},
  journal={IEEE Transactions on Human Factors in Electronics},
  number={1},
  pages={2--5},
  year={1964},
  publisher={IEEE}
}

% @article{recchiuto2016visual,
%   title={Visual feedback with multiple cameras in a UAVs Human--Swarm Interface},
%   author={Recchiuto, Carmine Tommaso and Sgorbissa, Antonio and Zaccaria, Renato},
%   journal={Robotics and Autonomous Systems},
%   volume={80},
%   pages={43--54},
%   year={2016},
%   publisher={Elsevier}
% }

% McRuer's crossover model
@article{mcruer1967review,
  title={A review of quasi-linear pilot models},
  author={McRuer, Duane T and Jex, Henry R},
  journal={IEEE transactions on human factors in electronics},
  number={3},
  pages={231--249},
  year={1967},
  publisher={IEEE}
}

%Human as observer, using McRuer's model
@article{van2015empirical,
  title={An empirical human controller model for preview tracking tasks},
  author={van der El, Kasper and Pool, Daan M and Damveld, Herman J and van Paassen, Marinus Ren{\'e} M and Mulder, Max},
  journal={IEEE transactions on cybernetics},
  volume={46},
  number={11},
  pages={2609--2621},
  year={2015},
  publisher={IEEE}
}

@article{hess2012modeling,
  title={Modeling the pilot detection of time-varying aircraft dynamics},
  author={Hess, Ronald A},
  journal={Journal of aircraft},
  volume={49},
  number={6},
  pages={2100--2104},
  year={2012}
}

@inproceedings{hess2011preliminary,
  title={A preliminary study of human pilot dynamics in the control of time-varying systems},
  author={Hess, Ronald},
  booktitle={AIAA modeling and simulation technologies conference},
  pages={6554},
  year={2011}
}

@article{drop2013identification,
  title={Identification of the feedforward component in manual control with predictable target signals},
  author={Drop, Frank M and Pool, Daan M and Damveld, Herman J and van Paassen, Marinus M and Mulder, Max},
  journal={IEEE transactions on cybernetics},
  volume={43},
  number={6},
  pages={1936--1949},
  year={2013},
  publisher={IEEE}
}
@article{van2010optimization,
  title={Optimization of human perception modeling using interval analysis},
  author={Van Kampen, E and Zaal, PMT and Weerdt, E de and Chu, QP and Mulder, JA},
  journal={Journal of guidance, control, and dynamics},
  volume={33},
  number={1},
  pages={42--52},
  year={2010}
}

@inproceedings{zaal2008new,
  title={New types of target inputs for multi-modal pilot model identification},
  author={Zaal, Peter and Pool, Daan and Mulder, M and van Paassen, M},
  booktitle={AIAA modeling and simulation technologies conference and exhibit},
  pages={7106},
  year={2008}
}






@article{kleinman1970optimal,
  title={An optimal control model of human response part I: Theory and validation},
  author={Kleinman, David L and Baron, S and Levison, WH},
  journal={Automatica},
  volume={6},
  number={3},
  pages={357--369},
  year={1970},
  publisher={Elsevier}
}



% Bringing the story together
@article{queralta2020collaborative,
  title={Collaborative multi-robot search and rescue: Planning, coordination, perception, and active vision},
  author={Queralta, Jorge Pena and Taipalmaa, Jussi and Pullinen, Bilge Can and Sarker, Victor Kathan and Gia, Tuan Nguyen and Tenhunen, Hannu and Gabbouj, Moncef and Raitoharju, Jenni and Westerlund, Tomi},
  journal={Ieee Access},
  volume={8},
  pages={191617--191643},
  year={2020},
  publisher={IEEE}
}



%Interesting similar theory
@article{mccord1991input,
  title={Input-versus output-oriented instructions on a compensatory tracking task: support for control theory},
  author={McCord, David M},
  journal={The Psychological Record},
  volume={41},
  pages={401--413},
  year={1991},
  publisher={Springer}
}

% survey which includes different control models of human behavior 
@article{scibilia2022human,
  title={Human control model estimation in physical human--machine interaction: A survey},
  author={Scibilia, Adriano and Pedrocchi, Nicola and Fortuna, Luigi},
  journal={Sensors},
  volume={22},
  number={5},
  pages={1732},
  year={2022},
  publisher={MDPI}
}


% 3d recontruction for situational/spatial awareness

@inproceedings{li2015flying,
  title={Flying frustum: A spatial interface for enhancing human-uav awareness},
  author={Li, Nico and Cartwright, Stephen and Shekhar Nittala, Aditya and Sharlin, Ehud and Costa Sousa, Mario},
  booktitle={Proceedings of the 3rd International Conference on Human-Agent Interaction},
  pages={27--31},
  year={2015}
}

% justification first person piloting challenges
%couples drones
@inproceedings{temma2019third,
  title={Third-person piloting: Increasing situational awareness using a spatially coupled second drone},
  author={Temma, Ryotaro and Takashima, Kazuki and Fujita, Kazuyuki and Sueda, Koh and Kitamura, Yoshifumi},
  booktitle={Proceedings of the 32nd Annual ACM Symposium on User Interface Software and Technology},
  pages={507--519},
  year={2019}
}

% control model--- human with memory
@article{martinez2017extended,
  title={Extended crossover model for human-control of fractional order plants},
  author={Mart{\'\i}nez-Garc{\'\i}a, Miguel and Gordon, Timothy and Shu, Lei},
  journal={IEEE Access},
  volume={5},
  pages={27622--27635},
  year={2017},
  publisher={IEEE}
}


@article{parker2017perceptual,
  title={Perceptual control models of pursuit manual tracking demonstrate individual specificity and parameter consistency},
  author={Parker, Maximilian G and Tyson, Sarah F and Weightman, Andrew P and Abbott, Bruce and Emsley, Richard and Mansell, Warren},
  journal={Attention, Perception, \& Psychophysics},
  volume={79},
  pages={2523--2537},
  year={2017},
  publisher={Springer}
}

@article{wewerinke1983model,
  title={Model of the human observer and decision maker—Theory and validation},
  author={Wewerinke, Paul H},
  journal={Automatica},
  volume={19},
  number={6},
  pages={693--696},
  year={1983},
  publisher={Elsevier}
}


@article{merat2012highly,
  title={Highly automated driving, secondary task performance, and driver state},
  author={Merat, Natasha and Jamson, A Hamish and Lai, Frank CH and Carsten, Oliver},
  journal={Human factors},
  volume={54},
  number={5},
  pages={762--771},
  year={2012},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}


%efference copy
@article{bridgeman2007efference,
  title={Efference copy and its limitations},
  author={Bridgeman, Bruce},
  journal={Computers in biology and medicine},
  volume={37},
  number={7},
  pages={924--929},
  year={2007},
  publisher={Elsevier}
}

@article{feldman2016active,
  title={Active sensing without efference copy: referent control of perception},
  author={Feldman, Anatol G},
  journal={Journal of neurophysiology},
  volume={116},
  number={3},
  pages={960--976},
  year={2016},
  publisher={American Physiological Society Bethesda, MD}
}
@book{chakraborty2014biologically,
  title={A Biologically Inspired Active Vision Framework for Cognitive Agents},
  author={Chakraborty, Arpan},
  year={2014},
  publisher={North Carolina State University}
}

% Very cool paper, if somewhat unrelated
@article{abadia2021cerebellar,
  title={A cerebellar-based solution to the nondeterministic time delay problem in robotic control},
  author={Abad{\'\i}a, Ignacio and Naveros, Francisco and Ros, Eduardo and Carrillo, Richard R and Luque, Niceto R},
  journal={Science Robotics},
  volume={6},
  number={58},
  pages={eabf2756},
  year={2021},
  publisher={American Association for the Advancement of Science}
}
@article{alkowatly2015bioinspired,
  title={Bioinspired autonomous visual vertical control of a quadrotor unmanned aerial vehicle},
  author={Alkowatly, Mohamad T and Becerra, Victor M and Holderbaum, William},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={38},
  number={2},
  pages={249--262},
  year={2015},
  publisher={American Institute of Aeronautics and Astronautics}
}

%Tracking a Maneuvering Target Using Input
Estimation Versus the Interacting Multiple Model
Algorithm
@article{bar1989tracking,
  title={Tracking a maneuvering target using input estimation versus the interacting multiple model algorithm},
  author={Bar-Shalom, Yaakov and Chang, Kevin C and Blom, Henk AP},
  journal={IEEE Transactions on Aerospace and Electronic Systems},
  volume={25},
  number={2},
  pages={296--300},
  year={1989},
  publisher={IEEE}
}

@article{floquet2006state,
  title={State and unknown input estimation for linear discrete-time systems},
  author={Floquet, Thierry and Barbot, Jean-Pierre},
  journal={Automatica},
  volume={42},
  number={11},
  pages={1883--1889},
  year={2006},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Takeover requests
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@inproceedings{ludwig2018comparison,
  title={A comparison of concepts for control transitions from automation to human},
  author={Ludwig, Julian and Haas, Andreas and Flad, Michael and Hohmann, Soren},
  booktitle={2018 IEEE International Conference on Systems, Man, and Cybernetics (SMC)},
  pages={3201--3206},
  year={2018},
  organization={IEEE}
}

@article{zeeb2015determines,
  title={What determines the take-over time? An integrated model approach of driver take-over after automated driving},
  author={Zeeb, Kathrin and Buchner, Axel and Schrauf, Michael},
  journal={Accident analysis \& prevention},
  volume={78},
  pages={212--221},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{gold2013take,
  title={“Take over!” How long does it take to get the driver back into the loop?},
  author={Gold, Christian and Damb{\"o}ck, Daniel and Lorenz, Lutz and Bengler, Klaus},
  booktitle={Proceedings of the human factors and ergonomics society annual meeting},
  volume={57},
  number={1},
  pages={1938--1942},
  year={2013},
  organization={Sage Publications Sage CA: Los Angeles, CA}
}

@article{morales2020automated,
  title={Automated driving: A literature review of the take over request in conditional automation},
  author={Morales-Alvarez, Walter and Sipele, Oscar and L{\'e}beron, R{\'e}gis and Tadjine, Hadj Hamma and Olaverri-Monreal, Cristina},
  journal={Electronics},
  volume={9},
  number={12},
  pages={2087},
  year={2020},
  publisher={MDPI}
}
@article{zeeb2015determines,
  title={What determines the take-over time? An integrated model approach of driver take-over after automated driving},
  author={Zeeb, Kathrin and Buchner, Axel and Schrauf, Michael},
  journal={Accident analysis \& prevention},
  volume={78},
  pages={212--221},
  year={2015},
  publisher={Elsevier}
}
@article{worle2020sleep,
  title={Sleep in highly automated driving: Takeover performance after waking up},
  author={W{\"o}rle, Johanna and Metz, Barbara and Othersen, Ina and Baumann, Martin},
  journal={Accident Analysis \& Prevention},
  volume={144},
  pages={105617},
  year={2020},
  publisher={Elsevier}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Haptics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Situational Awareness Haptics

@inproceedings{fink2023expanded,
  title={Expanded Situational Awareness Without Vision: A Novel Haptic Interface for Use in Fully Autonomous Vehicles},
  author={Fink, Paul DS and Abou Allaban, Anas and Atekha, Omoruyi E and Perry, Raymond J and Sumner, Emily S and Corey, Richard R and Dimitrov, Velin and Giudice, Nicholas A},
  booktitle={Proceedings of the 2023 ACM/IEEE International Conference on Human-Robot Interaction},
  pages={54--62},
  year={2023}
}
@article{gibbs2022comparison,
  title={A comparison of the effects of haptic and visual feedback on presence in virtual reality},
  author={Gibbs, Janet K and Gillies, Marco and Pan, Xueni},
  journal={International Journal of Human-Computer Studies},
  volume={157},
  pages={102717},
  year={2022},
  publisher={Elsevier}
}
% Situational awareness and haptics 
@inproceedings{teo2021impact,
  title={The Impact of a Synthetic Teammate on Situational Awareness},
  author={Teo, Aaron and Fieldhouse, Kenneth and Niemczyk, Mary},
  booktitle={87th International Symposium on Aviation Psychology},
  pages={178},
  year={2021}
}
% Haptic feedback for teleoperation
@article{son2013human,
  title={Human-centered design and evaluation of haptic cueing for teleoperation of multiple mobile robots},
  author={Son, Hyoung Il and Franchi, Antonio and Chuang, Lewis L and Kim, Junsuk and Bulthoff, Heinrich H and Giordano, Paolo Robuffo},
  journal={IEEE transactions on cybernetics},
  volume={43},
  number={2},
  pages={597--609},
  year={2013},
  publisher={IEEE}
}

@inproceedings{son2011evaluation,
  title={An evaluation of haptic cues on the tele-operator's perceptual awareness of multiple UAVs' environments},
  author={Son, Hyoung Il and Kim, Junsuk and Chuang, Lewis and Franchi, Antonio and Giordano, Paolo Robuffo and Lee, Dongjun and B{\"u}lthoff, Heinrich H},
  booktitle={2011 IEEE World Haptics Conference},
  pages={149--154},
  year={2011},
  organization={IEEE}
}

@inproceedings{son2011measuring,
  title={Measuring an operator's maneuverability performance in the haptic teleoperation of multiple robots},
  author={Son, Hyoung Il and Chuang, Lewis L and Franchi, Antonio and Kim, Junsuk and Lee, Dongjun and Lee, Seong-Whan and B{\"u}lthoff, Heinrich H and Giordano, Paolo Robuffo},
  booktitle={2011 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={3039--3046},
  year={2011},
  organization={IEEE}
}
@article{ni2018point,
  title={Point cloud augmented virtual reality environment with haptic constraints for teleoperation},
  author={Ni, Dejing and Nee, Andrew YC and Ong, Soh-Khim and Li, Huijun and Zhu, Chengcheng and Song, Aiguo},
  journal={Transactions of the Institute of Measurement and Control},
  volume={40},
  number={15},
  pages={4091--4104},
  year={2018},
  publisher={SAGE Publications Sage UK: London, England}
}


@inproceedings{zhang2021haptic,
  title={Haptic feedback improves human-robot agreement and user satisfaction in shared-autonomy teleoperation},
  author={Zhang, Dawei and Tron, Roberto and Khurshid, Rebecca P},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3306--3312},
  year={2021},
  organization={IEEE}
}

@inproceedings{selvaggio2019passive,
  title={Passive task-prioritized shared-control teleoperation with haptic guidance},
  author={Selvaggio, Mario and Giordano, P Robuffo and Ficuciello, Fanny and Siciliano, Bruno},
  booktitle={2019 international conference on robotics and automation (ICRA)},
  pages={430--436},
  year={2019},
  organization={IEEE}
}

@article{mohammadi2021aerial,
  title={Aerial tele-manipulation with passive tool via parallel position/force control},
  author={Mohammadi, Mostafa and Bicego, Davide and Franchi, Antonio and Barcelli, Davide and Prattichizzo, Domenico},
  journal={Applied Sciences},
  volume={11},
  number={19},
  pages={8955},
  year={2021},
  publisher={MDPI}
}
@article{van2020design,
  title={Design of a haptic feedback system for flight envelope protection},
  author={Van Baelen, Dirk and Ellerbroek, Joost and Van Paassen, MM and Mulder, Max},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={43},
  number={4},
  pages={700--714},
  year={2020},
  publisher={American Institute of Aeronautics and Astronautics}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Observer Models for Humans
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% From Controls Lit
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@inproceedings{radke2006survey,
  title={A survey of state and disturbance observers for practitioners},
  author={Radke, Aaron and Gao, Zhiqiang},
  booktitle={2006 American Control Conference},
  pages={6--pp},
  year={2006},
  organization={IEEE}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% From HRI Lit 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{baron1969human,
  title={The human as an optimal controller and information processor},
  author={Baron, Sheldon and Kleinman, David L},
  journal={IEEE Transactions on Man-Machine Systems},
  volume={10},
  number={1},
  pages={9--17},
  year={1969},
  publisher={IEEE}
}


@article{bao1989discrete,
  title={A Discrete Optimal Control Model of Human Response},
  author={Bao-Sheng, Hu and Zhi-Qiang, Liu},
  journal={IFAC Proceedings Volumes},
  volume={22},
  number={12},
  pages={95--98},
  year={1989},
  publisher={Elsevier}
}
@inproceedings{baron1976effects,
  title={The effects of deviate internal representations in the optimal model of the human operator},
  author={Baron, Sheldon and Berliner, Jeffrey E},
  booktitle={1976 IEEE Conference on Decision and Control including the 15th Symposium on Adaptive Processes},
  pages={1055--1057},
  year={1976},
  organization={IEEE}
}
@incollection{pew1978components,
  title={The components of an information processing theory of skilled performance based on an optimal control perspective},
  author={Pew, Richard W and Baron, Sheldon},
  booktitle={Information processing in motor control and learning},
  pages={71--78},
  year={1978},
  publisher={Elsevier}
}

@article{laquitaine2018switching,
  title={A switching observer for human perceptual estimation},
  author={Laquitaine, Steeve and Gardner, Justin L},
  journal={Neuron},
  volume={97},
  number={2},
  pages={462--474},
  year={2018},
  publisher={Elsevier}
}

@article{neilson1988internal,
  title={Internal models and intermittency: A theoretical account of human tracking behavior},
  author={Neilson, PD and Neilson, MD and O'dwyer, NJ},
  journal={Biological cybernetics},
  volume={58},
  pages={101--112},
  year={1988},
  publisher={Springer}
}

@article{vul2009explaining,
  title={Explaining human multiple object tracking as resource-constrained approximate inference in a dynamic probabilistic model},
  author={Vul, Ed and Alvarez, George and Tenenbaum, Joshua and Black, Michael},
  journal={Advances in neural information processing systems},
  volume={22},
  year={2009}
}

@article{baron1969human,
  title={The human as an optimal controller and information processor},
  author={Baron, Sheldon and Kleinman, David L},
  journal={IEEE Transactions on Man-Machine Systems},
  volume={10},
  number={1},
  pages={9--17},
  year={1969},
  publisher={IEEE}
}

@article{selva2012relationships,
  title={Relationships between Observer and Kalman filter models for human dynamic spatial orientation},
  author={Selva, Pierre and Oman, Charles M},
  journal={Journal of Vestibular Research},
  volume={22},
  number={2-3},
  pages={69--80},
  year={2012},
  publisher={IOS Press}
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{bentinck2022identifying,
  title={Identifying Human Preview Control Behavior Using Subsystem Identification},
  author={Bentinck, Pieter-Bas JC and Pool, Daan M and van der El, Kasper and Hoagg, Jesse B and Mulder, Max},
  journal={IFAC-PapersOnLine},
  volume={55},
  number={29},
  pages={172--177},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{mousavi2018effects,
  title={Effects of System Time Delay as Humans Learn to Control Dynamic Systems},
  author={Mousavi, S Alireza Seyyed and Hellstrom, Erik and Jankovic, Mrdjan and Santillo, Mario A and Seigler, TM and Hoagg, Jesse B},
  booktitle={2018 IEEE International Conference on Systems, Man, and Cybernetics (SMC)},
  pages={3446--3451},
  year={2018},
  organization={IEEE}
}

@article{koushkbaghi2022modeling,
  title={Modeling Human Control Behavior in Command-following Tasks},
  author={Koushkbaghi, Sajad},
  year={2022}
}

@article{peterson2022assessing,
  title={Assessing Human Feedback Parameters for Disturbance-Rejection},
  author={Peterson, Lauren N and Chou, Amber HY and Burden, Samuel A and Yamagami, Momona},
  journal={IFAC-PapersOnLine},
  volume={55},
  number={41},
  pages={1--6},
  year={2022},
  publisher={Elsevier}
}

@article{koushkbaghi2021impact,
  title={The impact of static output nonlinearities on the control strategies that humans use in command-following tasks},
  author={Koushkbaghi, Sajad and Hoagg, Jesse B and Seigler, T Michael},
  journal={Journal of the Franklin Institute},
  volume={358},
  number={6},
  pages={2964--2986},
  year={2021},
  publisher={Elsevier}
}

@article{yamagami2019contributions,
  title={Contributions of feedforward and feedback control in a manual trajectory-tracking task},
  author={Yamagami, Momona and Howell, Darrin and Roth, Eatai and Burden, Samuel A},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={34},
  pages={61--66},
  year={2019},
  publisher={Elsevier}
}

@article{yamagami2021effect,
  title={Effect of handedness on learned controllers and sensorimotor noise during trajectory-tracking},
  author={Yamagami, Momona and Peterson, Lauren N and Howell, Darrin and Roth, Eatai and Burden, Samuel A},
  journal={IEEE Transactions on Cybernetics},
  year={2021},
  publisher={IEEE}
}

@article{mousavi2020impact,
  title={The impact of command-following task on human-in-the-loop control behavior},
  author={Mousavi, S Alireza Seyyed and Matveeva, Faina and Zhang, Xingye and Seigler, T Michael and Hoagg, Jesse B},
  journal={IEEE Transactions on Cybernetics},
  volume={52},
  number={7},
  pages={6447--6461},
  year={2020},
  publisher={IEEE}
}
@article{zhang2020impact,
  title={The impact of nonminimum-phase zeros on human-in-the-loop control systems},
  author={Zhang, Xingye and Seigler, T Michael and Hoagg, Jesse B},
  journal={IEEE Transactions on Cybernetics},
  volume={52},
  number={6},
  pages={5098--5112},
  year={2020},
  publisher={IEEE}
}
@article{mousavi2021characteristics,
  title={Characteristics that make linear time-invariant dynamic systems difficult for humans to control},
  author={Mousavi, Seyyed Alireza Seyyed and Zhang, Xingye and Seigler, T Michael and Hoagg, Jesse B},
  journal={IEEE Transactions on Human-Machine Systems},
  volume={51},
  number={2},
  pages={141--151},
  year={2021},
  publisher={IEEE}
}

@inproceedings{yamagami2020decoding,
  title={Decoding intent with control theory: comparing muscle versus manual interface performance},
  author={Yamagami, Momona and Steele, Katherine M and Burden, Samuel A},
  booktitle={Proceedings of the 2020 CHI conference on human factors in computing systems},
  pages={1--12},
  year={2020}
}

@article{mabrok2020human,
  title={Human models in human-in-the-loop control systems},
  author={Mabrok, Mohamed A and Mohamed, Hassan K and Abdel-Aty, Abdel-Haleem and Alzahrani, Ahmed S},
  journal={Journal of Intelligent \& Fuzzy Systems},
  volume={38},
  number={3},
  pages={2611--2622},
  year={2020},
  publisher={IOS Press}
}

@article{zhang2017roles,
  title={The roles of feedback and feedforward as humans learn to control unknown dynamic systems},
  author={Zhang, Xingye and Wang, Shaoqian and Hoagg, Jesse B and Seigler, T Michael},
  journal={IEEE transactions on cybernetics},
  volume={48},
  number={2},
  pages={543--555},
  year={2017},
  publisher={IEEE}
}

@article{wewerinke1983model,
  title={Model of the human observer and decision maker—Theory and validation},
  author={Wewerinke, Paul H},
  journal={Automatica},
  volume={19},
  number={6},
  pages={693--696},
  year={1983},
  publisher={Elsevier}
}

@inproceedings{yu2014human,
  title={Human control strategies in pursuit tracking with a disturbance input},
  author={Yu, Bo and Gillespie, R Brent and Freudenberg, James S and Cook, Jeffrey A},
  booktitle={53rd IEEE Conference on Decision and Control},
  pages={3795--3800},
  year={2014},
  organization={IEEE}
}
